Measurement of the Spin of the Xi(1530) Resonance

The properties of the Xi(1530) resonance are investigated in the Lambdac+ --> Xi- pi+ K+ decay process. The data sample was collected with the BaBar detector at the SLAC PEP-II asymmetric-energy e+ e- collider operating at center of mass energies 10.58 and 10.54 GeV. The corresponding integrated luminosity is approximately 230 inverse fb. The spin of the Xi(1530) is established to be 3/2. The existence of an S-wave amplitude in the Xi- pi+ system is inferred, and its interference with the Xi(1530)0 amplitude provides the first clear demonstration of the Breit-Wigner phase motion expected for the Xi(1530). The P_1(cos[theta(Xi-)]) Legendre polynomial moment indicates the presence of a significant S-wave amplitude for Xi- pi+ mass values above 1.6 GeV/c^2, and a dip in the mass distribution at approximately 1.7 GeV/c^2 is interpreted as due to coherent addition of a Xi(1690)0 contribution to this amplitude. This would imply J^P=1/2^- for the Xi(1690). Attempts at fitting the Xi(1530)0 lineshape yield unsatisfactory results, and this failure is attributed to interference effects associated with the amplitudes describing the K+ pi+ and/or Xi- K+ systems.

==> abstract.tex <==
The properties of the $\Xi(1530)$ resonance are investigated in the $\Lambda_c^+\rightarrow \Xi^- \pi^+ K^+$ decay process.
The data sample was collected with the BaBar detector at the SLAC PEP-II asymmetric-energy $e^+ e^-$ collider operating at center
of mass energies 10.58 and 10.54 GeV. The corresponding integrated luminosity is approximately 230 fb$^{-1}$.
The spin of the $\Xi(1530)$ is established to be 3/2.  The existence of an $S$-wave amplitude in the $\Xi^- \pi^+$ system is inferred, 
and its interference with the $\Xi(1530)^0$ amplitude provides the first clear demonstration of the Breit-Wigner phase motion
expected for the $\Xi(1530)$.  The $P_1(\rm cos\,\theta_{\Xi^-})$ Legendre polynomial moment indicates the presence of a significant 
$S$-wave amplitude for $\Xi^- \pi^+$ mass values above 1.6 GeV/c$^2$, and a dip in the mass distribution at approximately 1.7 GeV/c$^2$ 
is interpreted as due to coherent addition of a $\Xi(1690)^0$ contribution to this amplitude.  This would imply $J^P=1/2^-$ for the 
$\Xi(1690)$.  Attempts at fitting the $\Xi(1530)^0$ lineshape yield unsatisfactory results, and this failure is attributed to 
interference effects associated with the amplitudes describing the $K^+ \pi^+$ and/or $\Xi^- K^+$ systems.



==> minisym.tex <==
\RequirePackage{xspace}

\usepackage{relsize}

\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\pep2{PEP-II}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}

